Transverse Energy Measurement and Fluctuation Studies in Ultra-Relativistic Heavy Ion Collisions

Transverse energy ($E_T$) has been measured with both of it's components, namely hadronic ($E_T^{had}$) and electromagnetic ($E_T^{em}$) at mid-rapidity, for 62.4 GeV Au+Au collisions by the STAR experiment. In the common phase space of TPC and BEMC ($0 < \eta < 1$ and full $\phi$), we have obtained $E_T^{had}$ from the TPC reconstructed tracks and $E_T^{em}$ from the BEMC tower hits after correcting for the hadronic contaminations in the calorimeter. The centrality behavior of $<dE_T/d\eta>/(0.5 N_{part})$ and the excitation function of $<dE_T/dy>/(0.5 N_{part})$ has been compared with the final state gluon saturation model (EKRT) along with similar measurements from SPS to RHIC. The most striking feature is the observation of a nearly constant value of $E_T/N_{ch} \sim 0.8$ GeV from AGS, SPS to RHIC. The $E_T$ and $N_{ch}$ production has been observed to follow a logarithmic behavior. The initial energy density estimated by the boost-invariant Bjorken hydrodynamic model, is well above the lattice QCD value for a deconfined matter of Quarks and Gluons. Taking similar colliding species i.e. Au+Au, the $\epsilon_{Bj} .\tau$ has been predicted for LHC, based on the measurements at RHIC. We have also made predictions for $(dE_T/d\eta)/(0.5 N_{part})$ and $(dN_{ch}/d\eta)/(0.5 N_{part})$ for the LHC energy. Furthermore, we have studied the event-by event fluctuations in $E_T$ and in the ratio of it's components using $\sigma/\mu$ as the fluctuation observable.

==> ref_1.tex <==
\begin{thebibliography}{99}
\bibitem{collins} J.C. Collins and M.J. Perry, \prl{\bf 34} (1975) 1353.
\bibitem{qcdPhase} P. Braun-Munzinger, \npa{\bf 681} (2001) 119c.
\bibitem{karsch} F. Karsch, Lect.Notes Phys.{\bf 583} (2002) 209-249.
\bibitem{halzen} F. Halzen and H.C. Liu, \prd{\bf 25} (1982) 1842.
\bibitem{shuryak} E.V. Shuryak, \pr{\bf 61} (1980) 71.
\bibitem{gavai}  J. Cleymans, R.V. Gavai and E. Suhonen, \pr{\bf 130} (1986) 217.
\bibitem{cpSingh}  C.P. Singh, \pr{\bf 236} (1993) 147-224.
\bibitem{kajantieM}  K.Kajantie and L. McLerran, Annu. Rev. Nucl. Part. Sci.{\bf 37} (1987) 293.
\bibitem{bass}  S.A. Bass {\it et al.}, \jpg{\bf 25} (1999) R1-R57.
\bibitem{muller} Berndt Muller, \rpp{\bf 58} (1995) 611-636.
\bibitem{rafel}  J.Rafelski and B. Muller, \prl{\bf 48} (1982) 1066.
\bibitem{pkoch}  P.Koch, B. Muller and J.Rafelski, \pr{\bf 142} (1986) 165.
\bibitem{manuel} M. Calderon de la Barca Sanchez, Ph.D. thesis, Yale University, USA, 2001.
\bibitem{odyniec} G. Odyniec, \npa{\bf 681} (2001) 197c-204c.
\bibitem{matsui} T. Matsui and H. Satz, \plb{\bf 178} (1986) 416.
\bibitem{na38} C. Baglin {\it et al.}, NA38 collaboration \plb{\bf 220} (1989) 471, 
  \plb{\bf 251} (1990) 465, \plb{\bf 251} (1990) 472, \plb{\bf 255} (1991) 459, 
  \plb{\bf 268} (1991) 453, \plb{\bf 270} (1991) 105, \plb{\bf 272} (1991) 449.
\bibitem{na50} M. Gonin {\it et al.}, \npa{\bf 610} (1996) 404c.
\bibitem{na50_1} M.C. Abreu {\it et al.}, \npa{\bf 661} (1999) 93.
\bibitem{na50_2} M.C. Abreu {\it et al.}, \plb{\bf 447} (2000) 28.
\bibitem{rhic_jpsi} R.L. Thews {\it et al.}, \prc{\bf 63} (2001) 054905.
\bibitem{phenixJ} S.S. Adler {\it et al.}, PHENIX collaboration \prc{\bf 69} (2004) 014901.
\bibitem{capella} A. Capella {\it et al.}, \prl{\bf 85} (2000) 2080.
\bibitem{eLoss} X.N. Wang and M. Gyulassy, \prl{\bf 68} (1992) 1480.
\bibitem{starJet} J. Adams {\it et al.}, STAR Collaboration \prl{\bf 93} (2004) 252301.
\bibitem{sinha} S. Raha and B. Sinha, \ijmpa{\bf 6} (1991) 517.
\bibitem{kapu} K. Kajantie {\it et al.}, \prd{\bf 34} (1986) 2746.
\bibitem{jkapu} J. Kapusta {\it et al.}, \prd{\bf 44} (1991) 2774, (erratum 
  \prd{\bf 47} (1993) 4171.
\bibitem{dks} D.K. Srivastava {\it et al.}, \plb{\bf 276} (1992) 285.
\bibitem{strick} M. Strickland, \plb{\bf 331} (1994) 245.
\bibitem{wa98} M.M. Aggarwal {\it et al.}, WA98 Collaboration \prl{\bf 85} (2000) 3595.
\bibitem{phenixDPp} S.S. Adler {\it et al.}, PHENIX Collaboration \prd{\bf 71} (2005) 071102(R).
\bibitem{phenixDPA} S.S. Adler {\it et al.}, PHENIX Collaboration \prl{\bf 94} (2005) 232301.
\bibitem{ceres1} T. Ullrich {\it et al.}, \npa{\bf 610} (1996) 317c.
\bibitem{ceres2} A. Drees, \npa{\bf 610} (1996) 536c.
\bibitem{hydroQGP} D.K. Srivastava {\it et al.}, \npa{\bf 610} (1996) 350c.
\bibitem{rapp} R. Rapp {\it et al.}, \npa{\bf 617} (1997) 472.
\bibitem{zxu} Z. Xu, \jpg{\bf 30} (2004) S325.
\bibitem{kapusta} J. Kapusta {\it et al.}, \plb{\bf 163} (1985) 253.
\bibitem{gersdorff} H. v Gersdorff, \npa{\bf 461} (1987) 251c.
\bibitem{hoffman} J. Hofmann {\it et al.}, \prl{\bf 36} (1976) 88.
\bibitem{stocker} H. Stocker and W. Greiner, \pr{\bf 137} (1986) 277.
\bibitem{amelin} N.S. Amelin {\it et al.}, \npa{\bf 544} (1992) 463c.
\bibitem{kataja} M. Kataja {\it et al.}, \prd{\bf 34} (1986) 2755.
\bibitem{vanHove} L. Van Hove, \plb{\bf 118} (1982) 138.
\bibitem{landau} L.D. Landau, {\it Izv. Akad. Nauk. SSSR Ser. Fiz.}{\bf 17} (1953) 51; collected
  papers Ed. by  D. Ter Haar (Pergamon, Oxford, 1965) p. 569.
\bibitem{sarkar} S. Sarkar {\it et al.}, \prc{\bf 51} (1995) 318.[Erratum:ibid {\bf C51} (1995) 2845.]
\bibitem{dumitru} A. Dumitru {\it et al.}, \zpa{\bf 353} (1995) 187.
\bibitem{flow130} K.H. Ackermann {\it et al.}, STAR Collaboration \prl{\bf 86} (2001) 402.
\bibitem{flow130I} C. Adler {\it et al.}, STAR Collaboration \prl{\bf 87} (2001) 182301.
\bibitem{flowMS} C. Adler {\it et al.}, STAR Collaboration \prl{\bf 89} (2002) 132301.
\bibitem{flowMS200} J. Adams {\it et al.}, STAR Collaboration \prl{\bf 95} (2005) 122301.
\bibitem{kharzeev} D. Kharzeev and M. Nardi, \plb{\bf 507} (2001) 121.
\bibitem{bernard} C. Bernard {\it et al.}, \prd{\bf 55} (1997) 6861; Y. Iwasaki {\it et al.},
  \prd{\bf 54} (1996) 7010.
\bibitem{boydG} G. Boyd {\it et al.}, \prl{\bf 75} (1995) 4169.
\bibitem{heiselberg} H. Heiselberg, \pr{\bf 351} (2001) 161 and the refernces therein.
\bibitem{jeon} S. Jeon and V. Koch, \prl{\bf 83} (1999) 5435.
\bibitem{jeon2} S. Jeon and V. Koch, \prl{\bf 85} (2000) 2076.
\bibitem{gavin} S. Gavin and C. Pruneau, nucl-th/9906060 and nucl-th/9907040.
\bibitem{netCh} J. Adams {\it et al.}, STAR Collaboration, \prc{\bf 68} (2003) 044905.
\bibitem{meanPt} J. Adams {\it et al.}, STAR Collaboration, \prc{\bf 71} (2005) 064906, 
  H. Appelhauser {\it et al.}, NA49 Collaboration \plb{\bf 459} (1999) 679.
\bibitem{etFluct} T. Akesson {\it et al.}, Helios Collaboration \zpc{\bf 38} (1988) 383,
  H. Heiselberg {\it et al.}, \prl{\bf 67} (1991) 2946,  B. Blattel {\it et al.}, 
  \npa{\bf 544} (1992) 479c.
\bibitem{sFluct} M.I. Gorenstein {\it et al.}, \plb{\bf 585} (2004) 237.
\bibitem{isospin} B. Mohanty and J. Serreau, \pr{\bf 414} (2005) 263.
  
\bibitem{bjorken} J.D. Bjorken, \prd{\bf 27} (1983) 140.
\bibitem{entropy} A. Krasnitz, Y. Nara, R. Venugopalan, \npa{\bf 717} (2003) 268.
\bibitem{hijing} M. Gyulassy and X.N. Wang, \cpc{\bf 83} (1994) 307.
\bibitem{lund} B. Andersson {\it et al.}, \pr{\bf 97} (1983) 31.


\end{thebibliography}

==> ref_2.tex <==
\begin{thebibliography}{99}
\bibitem{rhic} H. Hahn {\it et al}., \nima{\bf 499} (2003) 245-263.
\bibitem{star} K.H. Ackermann {\it et al}., \nima{\bf 499} (2003) 624-632.
\bibitem{phenix} K. Adcox {\it et al}., \nima{\bf 499} (2003) 469-479.
\bibitem{phobos} B.B. Back {\it et al}., \nima{\bf 499} (2003) 603-623.
\bibitem{brahms} M. Adamczyk {\it et al}., \nima{\bf 499} (2003) 437-468.
\bibitem{magnet} F. Bergsma {\it et al}., \nima{\bf 499} (2003) 629.
\bibitem{tpc} M. Anderson {\it et al}., \nima{\bf 499} (2003) 659-678.
\bibitem{bethe} W.R. Leo, Techniques for Nuclear and Particle Physics Experiments,
page 23-28, Narosa Publishing House.
\bibitem{svt} R. Bellwied {\it et al}., \nima{\bf 499} (2003) 640-651.
\bibitem{ssd} L. Arnold {\it et al}., \nima{\bf 499} (2003) 652-658.
\bibitem{ftpc} K.H. Ackermann {\it et al}., \nima{\bf 499} (2003) 713-719.
\bibitem{rich} STAR/ALICE RICH collaboration, a ring imaging cherenkov 
  detector for STAR, STARnote 349, 1998.
\bibitem{tof} B. Bonner {\it et al}., \nima{\bf 508} (2003) 181-184.
\bibitem{bemc} M. Beddo {\it et al}., \nima{\bf 499} (2003) 725-739.
\bibitem{eemc} C.E. Allgower {\it et al}., \nima{\bf 499} (2003) 740-750.
\bibitem{pmd} M.M. Aggarwal {\it et al}., \nima{\bf 499} (2003) 751-761.
\bibitem{pmdFlow} M.M. Aggarwal {\it et al}., \epjc{\bf 41} (2005) 287-296.	
\bibitem{bMohantyTH} B. Mohanty, Ph.D. Thesis, Institute of Physics, India, 2002.
\bibitem{pmdPRL} J. Adams {\it et al}., \prl{\bf 95} (2005) 062301.
\bibitem{gassiplex} J.C. Santiard, ALICE Internal Report, CERN-ECP/94-17.
\bibitem{fpd} {\it Proposal to Install a Forward Pion Detector in STAR},\\
``http://www.star.bnl.gov/STAR/html/$fpd\_l$/''.
\bibitem{ctb}  F.S. Bieser {\it et al}., \nima{\bf 499} (2003) 766.
\bibitem{zdc}  C. Adler {\it et al}., \nima{\bf 499} (2003) 433.



\end{thebibliography}

==> ref_3.tex <==
\begin{thebibliography}{99}
\bibitem{etGen} M. Jacob and P.V. Landshoff, \mpla{\bf 1} (1986) 657;
X.N. Wang, \pr{\bf 280} (1997) 287.
\bibitem{star200GeV} J. Adams {\it et al}., STAR Collaboration, \prc{\bf 70} (2004) 054907.
\bibitem{helios} T. Akesson {\it et al}., HELIOS Collaboration, \zpc{\bf 38} (1988) 383.
\bibitem{starSpectra} J. Adams {\it et al}., STAR Collaboration, Long \prc under preparation.
\bibitem{resolRef} J. Adams {\it et al}., STAR Collaboration, \plb {\bf 637} (2006) 161.
\bibitem{hijingPRD} X.N. Wang and M. Gyulassy, \prd {\bf 44} (1991) 3501.
\bibitem{abbott} T. Abbott {\it et al}., \prc{\bf 63} (2001) 064602.
\bibitem{bemcCalib} T. Cormier {\it et al}., \nima{\bf 483} (2002) 734.
\bibitem{hydro} P.F. Kolb {\it et al}., \npa{\bf 696} (2001) 197.
\bibitem{starPRL} J. Adams {\it et al}., STAR Collaboration, \prl{\bf 91} (2003) 172302.
\bibitem{kharzeevNpart} D. Kharzeev and M. Nardi, \plb{\bf 507} (2001) 121.
\bibitem{enterria} David d'Enterria, nucl-ex/0608049.
\bibitem{ekrt} K.J. Eskola {\it et al}., \npb{\bf 570} (2000) 379.
\bibitem{Barrettee} J. Barrettee {\it et al}., \prl{\bf 70} (1993) 2996.
\bibitem{Alber} T. Alber {\it et al}., \prl{\bf 75} (1995) 3814.
\bibitem{wa98Et} M.M. Aggarwal {\it et al}., WA98 Collaboration, \epjc{\bf 18} (2001) 651. 
\bibitem{phenixEt} K. Adcox {\it et al}., PHENIX Collaboration, \prl{\bf 87} (2001) 052301.
\bibitem{lnp} M. Gyulassy, {\it Lecture Notes in Physics} {\bf 583} (2001) 37.
\bibitem{phenixSyst} S.S. Adler {\it et al}., PHENIX Collaboration, \prc{\bf 71} (2005) 034908.
\bibitem{latticeQCD} F. Karsch, \npa{\bf 698} (2002) 199c.
\bibitem{eAuScatt} B. Hahn {\it et al}., \pr{\bf 101} (1956) 1131; C.W. De Jager {\it et al}.,
At. Data Nucl. Data Tables {\bf 24} (1974) 479;
\bibitem{hydro1} T.S. Ullrich, \npa{\bf 715} (2003) 399c.
\bibitem{hydro2} J. Adams {\it et al}., STAR Collaboration, \prl{\bf 92} (2004) 052302.
\bibitem{hydro3} P.F. Kolb and U. Heinz, nucl-th/0305084 (2003).
\bibitem{ags1} L. Ahle {\it et al}., E802 Collaboration, \prc{\bf 59} (1999) 2173.
\bibitem{ags2} L. Ahle {\it et al}., E802 Collaboration, \prc{\bf 58} (1998) 3523.
\bibitem{ags3} B.B. Back {\it et al}., E917 Collaboration, \prl{\bf 86} (2001) 1970.
\bibitem{ags4} L. Ahle {\it et al}., E802 Collaboration, \prc{\bf 57} (1998) 466(R).
\bibitem{na49-1} J. Bachler {\it et al}., NA49 Collaboration, \npa{\bf 661} (1999) 45.
\bibitem{na49-2} S.V. Afanasiev {\it et al}., NA49 Collaboration, \prc{\bf 66} (2002) 054902.
\bibitem{na49-3} M. van Leeuwen {\it et al}., NA49 Collaboration, \npa{\bf 715} (2003) 161.
\bibitem{fopi1} W. Reisdorf {\it et al}., FOPI Collaboration, \npa{\bf 612} (1997) 493.
\bibitem{fopi2} W. Reisdorf {\it et al}., FOPI Collaboration, \zpa{\bf 357} (1997) 215.
\bibitem{fopi3} B. Hong {\it et al}., FOPI Collaboration, \prc{\bf 66} (2002) 034901.
\bibitem{phenixPRC} S.S. Adler {\it et al}., PHENIX Collaboration, \prc{\bf 69} (2004) 034909.
\bibitem{wa80prc} R. Albrecht {\it et al}., WA80 Collaboration, \prc{\bf 44} (1991) 2736. 
\bibitem{wa98Syst} WA98 Collaboration, Systematics of Transverse Energy Production in
Pb+Pb Collisions at 158 GeV/nucleon (1996).
\bibitem{halzenF} F. Halzen and H.C. Liu, \prd{\bf 25} (1982) 1842.


\end{thebibliography}

==> ref_4.tex <==
\begin{thebibliography}{99}
\bibitem{fluctTherm} L. Van Hove, \plb{\bf 118} (1982) 138; H. Heiselberg,
\pr{\bf 351} (2001) 161; E.V. Shuryak, \plb{\bf 423} (1998) 9; S. Mrowczynski,
\prc{\bf 57} (1998) 1518; \plb{\bf 430} (1998) 9; M. Gazdzicki and S. Mrowczynski,
\zpc{\bf 57} (1992) 127.
\bibitem{QCDPhase} M. Stephanov {\it et al}., \prl{\bf 81} (1998) 4816;
\prd{\bf 60} (1999) 114028.
\bibitem{baymHH} G. Baym and H. Heiselberg, \plb{\bf 469} (1999) 7.
\bibitem{asakawaMuller} M. Asakawa {\it et al}., \prl{\bf 85} (2000) 2072.
\bibitem{jeonKoch} S. Jeon and V. Koch, \prl{\bf 83} (1999) 2076.
\bibitem{fluctMethods} C. Pruneau, {\it et al}., \prc{\bf 66} (2002) 044904.
\bibitem{droplet} L. van Hove, \zpc{\bf 21} (1984) 93; J.I. Kapusta and 
A.P. Vischer, \prc{\bf 52} (1995) 2725.
\bibitem{dcc1} M.M. Aggarwal {\it et al}., WA98 Collaboration, \prc{\bf 64} (2001) 
011901(R).
\bibitem{dcc2} B.Mohanty and J. Serreau, \pr{\bf 414} (2005) 263-358 and the
references therein. 
\bibitem{strange} M.I. Gorenstein {\it et al}., \plb{\bf 585} (2004) 237.
\bibitem{etJPsi} J.P. Blaizot {\it et al}., \prl{\bf 85} (2000) 4012.
\bibitem{gaussian} H. Appelshauser {\it et al}., NA49 Collaboration, \plb{\bf 459}
 (1999) 679; G. Roland, \npa{\bf 638} (1998) 91c.
\bibitem{phenixEtFluct} K. Adcox {\it et al}., PHENIX Collaboration, \prc{\bf 66}
 (2002) 024901.
\bibitem{baymFluct} G. Baym {\it et al}., \plb{\bf 219} (1989) 205.
\bibitem{rAlbrecht} R. Albrecht {\it et al}., \zpc{\bf 45} (1989) 31.
\bibitem{na34Fluct} F. Corriveau {\it et al}., NA34 Collaboration, \zpc{\bf 38} 
(1988) 15; J. Schukraft {\it et al}.,  NA34 Collaboration, \zpc{\bf 38} (1988) 59. 
\bibitem{phiMeasure} M. Gazdzicki and S. Mrowczynski, \zpc{\bf 54} (1992) 127.
\bibitem{balanceFn} S A. Bass {\it et al}., \prl{\bf 85} (2000) 2689.

\end{thebibliography}

==> ref_5.tex <==
\begin{thebibliography}{99}
\bibitem{elliptic} J. Adams {\it et al}., STAR Collaboration, \prl{\bf 92} (2004) 052302.
\bibitem{agreement} P.F. Kolb and U. Heinz, nucl-th/0305084 (2003).
\bibitem{supression} C. Adler {\it et al}., STAR Collaboration, \prl{\bf 89} (2002) 202301;
C. Adler {\it et al}., STAR Collaboration, \prl{\bf 90} (2003) 082302;
J. Adams {\it et al}., STAR Collaboration, \prl{\bf 91} (2003) 072304.

\end{thebibliography}
